Performance Modeling of Next-Generation Wireless Networks

The industry is satisfying the increasing demand for wireless bandwidth by densely deploying a large number of access points which are centrally managed, e.g. enterprise WiFi networks deployed in university campuses, companies, airports etc. This small cell architecture is gaining traction in the cellular world as well, as witnessed by the direction in which 4G+ and 5G standardization is moving. Prior academic work in analyzing such large-scale wireless networks either uses oversimplified models for the physical layer, or ignores other important, real-world aspects of the problem, like MAC layer considerations, topology characteristics, and protocol overhead. On the other hand, the industry is using for deployment purposes on-site surveys and simulation tools which do not scale, cannot efficiently optimize the design of such a network, and do not explain why one design choice is better than another. In this paper we introduce a simple yet accurate analytical model which combines the realism and practicality of industrial simulation tools with the ability to scale, analyze the effect of various design parameters, and optimize the performance of real- world deployments. The model takes into account all central system parameters, including channelization, power allocation, user scheduling, load balancing, MAC, advanced PHY techniques (single and multi user MIMO as well as cooperative transmission from multiple access points), topological characteristics and protocol overhead. The accuracy of the model is verified via extensive simulations and the model is used to study a wide range of real world scenarios, providing design guidelines on the effect of various design parameters on performance.

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_pics/antonios.JPG}}]{Antonios Michaloliakos}
graduated in 2009 from the department of Electrical and Computer Engineering of the National Technical University of Athens. He is currently pursuing a PhD in Electrical Engineering at the University of Southern California. His interests span the areas of probabilistic modeling and design of networks and cross-layer optimization in new generation wireless networks. He is currently working on developing a MAC protocol for a MU-MIMO system.
\end{IEEEbiography} 


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_pics/rrogalin.jpg}}]{Ryan Rogalin}
  received his BS degree in Electrical Engineering summa cum laude from the University of
  Oklahoma in 2008.  In 2010 he received his MS degree, also in Electrical Engineering, from the University of Southern California.
  He is currently a PhD student in
  Electrical Engineering at the University of Southern California as an Annenberg Fellow.  His research
  interests lie at the intersection of Communication Theory, Information Theory,
  wireless networks and their implementation through software defined radio.
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_pics/Yonglong.jpg}}]{Yonglong Zhang}
 graduated from the department of Electrical and Computer Engineering of the ƒcole SupŽrieure des Sciences et Technologies de l'IngŽnieur de Nancy in 2012. He is a PhD student in Electrical Engineering at the University of Southern California advised by Konstantinos Psounis. His research interests are performance analyzing of computer networks and WLAN resource management. He is currently working on user-AP association protocol for enterprise Wi-Fi networks.
\end{IEEEbiography} 


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_pics/psounis.jpg}}]{Konstantinos Psounis}
  is an Associate Professor of Electrical Engineering and Computer Science at the University of Southern California. He received his
  first degree from the department of Electrical and Computer Engineering of National Technical University of Athens, Greece, in June
  1997, and the M.S.and PhD degrees in Electrical Engineering from Stanford University, California, in January 1999 and December 2002
  respectively. Konstantinos models and analyzes the performance of a variety of wired and wireless networks. He also designs methods,
  algorithms, and protocols to solve problems related to such systems. He is a senior member of both IEEE and ACM.
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_pics/caire.jpg}}]{Giuseppe Caire}
(S '92 -- M '94 -- SM '03 -- F '05)
was born in Torino, Italy, in 1965. He received the B.Sc. in Electrical Engineering  from Politecnico di Torino (Italy), in 1990,
the M.Sc. in Electrical Engineering from Princeton University in 1992
and the Ph.D. from Politecnico di Torino in 1994.
He was a recipient of the AEI G.Someda Scholarship in 1991,
has been with the European Space Agency (ESTEC, Noordwijk, The Netherlands) from May 1994 to February 1995,
was a recipient of the COTRAO Scholarship in 1996 and of a CNR Scholarship in 1997.

%He has been visiting Princeton University in Summer 1997 and Sydney University  in Summer 2000.  He has been Assistant Professor in Telecommunications at the Politecnico di Torino, Associate Professor at the University of Parma, Italy,  Professor with the Department of Mobile Communications at the Eurecom Institute,  Sophia-Antipolis, France, and he is currently a professor of Electrical Engineering with the Viterbi School of Engineering, University of Southern California, Los Angeles, CA.

%He served as Associate Editor for the IEEE Transactions on Communications in 1998-2001 and as Associate Editor for the IEEE Transactions on Information Theory in 2001-2003.  He received the Jack Neubauer Best System Paper Award from the IEEE Vehicular Technology Society in 2003,  and the
%IEEE Communications Society \& Information Theory Society Joint Paper Award in 2004 and in 2011.
%Giuseppe Caire is Fellow of IEEE since 2005.  He has served in the Board of Governors of the IEEE Information Theory Society from 2004 to 2007,
%and as President of the  IEEE Information Theory Society in 2011.
%His main research interests are in the field of communications theory, information theory, channel and source coding
%with particular focus on wireless communications.
\end{IEEEbiography} 

